EMG-Based Adaptation of Anisotropic Virtual Fixtures for Robot-Assisted Surgical Resection and Dissection

In this paper, we address the development of an adaptive assistance system for robot-assisted laparoscopic surgery, specifically for delicate tasks such as Resection and Dissection. Even if Virtual Fixtures offer significant advantages for guiding a surgeon's movements, conventional Virtual Fixtures are often defined by fixed geometries, lacking the flexibility to adapt to the surgical workflow or the surgeon's immediate intent. To address these limitations, we propose a novel framework for an adaptive and anisotropic virtual fixture. In addition, we introduce an intuitive control interface that modulates the fixture's geometry in real-time based on the surgeon's intent, inferred from EMG signals. This approach allows the surgeon to dynamically expand or disengage the constraint by contracting their forearm muscles, enabling seamless transitions between precise guided motion and free repositioning of the tool. Experimental results from a pilot user study, based on a standardized surgical training task, demonstrate the effectiveness of the proposed method. The system showed significant improvements in task accuracy and movement consistency, alongside a reduction in perceived cognitive load, effort, and frustration.

==> mathbase.tex <==

\newcommand{\tras}{^{\mbox{\tiny T}}}
\newcommand{\mtras}{^{\mbox{\tiny -T}}}
\newcommand{\dtras}{^{\mbox{\tiny T}\dag}}
\newcommand{\muno}{^{\mbox{\tiny -1}}}
\newcommand{\tracon}{^{*}}
\newcommand{\mtracon}{^{-*}}
%\newcommand{\ds}{\displaystyle}
\newcommand{\ts}{\textstyle}
\newcommand{\scr}{\scriptstyle}
\newcommand{\sscr}{\scriptscriptstyle}
\newcommand{\bbar}[1]{\bar{\bar{#1}}}

 \newcommand{\evidenzia}[1]{\psframebox[framesep=5pt]{#1}}
 \newcommand{\BoxedEPSF}{\epsfbox} %% Primo capitolo
 \newcommand{\bo}{\mbox{\bf o}}
 \newcommand{\und}{\underline}
 \newcommand{\Span}{\mbox{\rm span}}
 \newcommand{\spann}{\mbox{\rm span}}
 \newcommand{\Agg}{\mbox{\rm agg}}
 \newcommand{\adj}{\mbox{\rm adj}}
 \newcommand{\Imm}{\mbox{\rm Im}}
 \newcommand{\Ker}{\mbox{\rm ker}}
 \newcommand{\rango}{\mbox{\rm rango}}
% \newcommand{\bM}{{\bf M}}
 \newcommand{\mat}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
 \newcommand{\mdet}[2]{\left|\begin{array}{#1} #2 \end{array}\right|}
 \newcommand{\cofbin}[2]{\left(\!\begin{array}{c}#1\\ #2 \end{array}\!\right)}

% Bold face:
\def\a{{\bf a}} \def\b{{\bf b}} \def\c{{\bf c}} \def\d{{\bf d}}
\def\e{{\bf e}} \def\f{{\bf f}} \def\g{{\bf g}} \def\h{{\bf h}}
\def\ib{{\bf i}} \def\j{{\bf j}} \def\k{{\bf k}} \def\l{{\bf l}}
\def\m{{\bf m}} \def\n{{\bf n}} \def\o{{\bf o}} \def\p{{\bf p}}
\def\q{{\bf q}} \def\r{{\bf r}} \def\s{{\bf s}} \def\t{{\bf t}}
\def\u{{\bf u}} \def\v{{\bf v}} \def\w{{\bf w}} \def\x{{\bf x}}
\def\y{{\bf y}} \def\z{{\bf z}}

\def\A{{\bf A}} \def\B{{\bf B}} \def\C{{\bf C}} \def\D{{\bf D}}
\def\E{{\bf E}} \def\F{{\bf F}} \def\G{{\bf G}} \def\H{{\bf H}}
\def\I{{\bf I}} \def\J{{\bf J}} \def\K{{\bf K}} \def\L{{\bf L}}
\def\M{{\bf M}} \def\N{{\bf N}} \def\O{{\bf O}} \def\P{{\bf P}}
\def\Q{{\bf Q}} \def\R{{\bf R}} \def\S{{\bf S}} \def\T{{\bf T}}
\def\U{{\bf U}} \def\V{{\bf V}} \def\W{{\bf W}} \def\X{{\bf X}}
\def\Y{{\bf Y}} \def\Z{{\bf Z}}

% Calligraphics:

\def\cA{{\cal A}} \def\cB{{\cal B}} \def\cC{{\cal C}} \def\cD{{\cal D}}
\def\cE{{\cal E}} \def\cF{{\cal F}} \def\cG{{\cal G}} \def\cH{{\cal H}}
\def\cI{{\cal I}} \def\cJ{{\cal J}} \def\cK{{\cal K}} \def\cL{{\cal L}}
\def\cM{{\cal M}} \def\cN{{\cal N}} \def\cO{{\cal O}} \def\cP{{\cal P}}
\def\cQ{{\cal Q}} \def\cR{{\cal R}} \def\cS{{\cal S}} \def\cT{{\cal T}}
\def\cU{{\cal U}} \def\cV{{\cal V}} \def\cW{{\cal W}} \def\cX{{\cal X}}
\def\cY{{\cal Y}} \def\cZ{{\cal Z}}

% tilde bold face:

\def\ta{\tilde{\a}} \def\tb{\tilde{\b}} \def\tc{\tilde{\c}}
\def\td{\tilde{\d}} \def\te{\tilde{\e}} \def\tf{\tilde{\f}}
\def\tg{\tilde{\g}} \def\th{\tilde{\h}} \def\tib{\tilde{\i}}
\def\tj{\tilde{\j}} \def\tk{\tilde{\k}} \def\tl{\tilde{\l}}
\def\tm{\tilde{\m}} \def\tn{\tilde{\n}} \def\to{\tilde{\o}}
\def\tp{\tilde{\p}} \def\tq{\tilde{\q}} \def\tr{\tilde{\r}}
\def\tts{\tilde{\s}} \def\ttt{\tilde{\t}} \def\tu{\tilde{\u}}
\def\tv{\tilde{\v}} \def\tw{\tilde{\w}} \def\tx{\tilde{\x}}
\def\ty{\tilde{\y}} \def\tz{\tilde{\z}}

\def\tA{\tilde{\A}} \def\tB{\tilde{\B}} \def\tC{\tilde{\C}}
\def\tD{\tilde{\D}} \def\tE{\tilde{\E}} \def\tF{\tilde{\F}}
\def\tG{\tilde{\G}} \def\tH{\tilde{\H}} \def\tI{\tilde{\I}}
\def\tJ{\tilde{\J}} \def\tK{\tilde{\K}} \def\tL{\tilde{\L}}
\def\tM{\tilde{\M}} \def\tN{\tilde{\N}} \def\tO{\tilde{\O}}
\def\tP{\tilde{\P}} \def\tQ{\tilde{\Q}} \def\tR{\tilde{\R}}
\def\tS{\tilde{\S}} \def\tT{\tilde{\T}} \def\tU{\tilde{\U}}
\def\tV{\tilde{\V}} \def\tW{\tilde{\W}} \def\tX{\tilde{\X}}
\def\tY{\tilde{\Y}} \def\tZ{\tilde{\Z}}

% Overline bold face:

\def\ooa{\overline{\a}} \def\oob{\overline{\b}}
\def\ooc{\overline{\c}} \def\ood{\overline{\d}}
\def\ooe{\overline{\e}} \def\oof{\overline{\f}}
\def\oog{\overline{\g}} \def\ooh{\overline{\h}}
\def\ooib{\overline{\ib}} \def\ooj{\overline{\j}}
\def\ook{\overline{\k}} \def\ool{\overline{\l}}
\def\oom{\overline{\m}} \def\oon{\overline{\n}}
\def\ooo{\overline{\o}} \def\oop{\overline{\p}}
\def\ooq{\overline{\q}} \def\oor{\overline{\r}}
\def\oos{\overline{\s}} \def\oot{\overline{\t}}
\def\oou{\overline{\u}} \def\oov{\overline{\v}}
\def\oow{\overline{\w}} \def\oox{\overline{\x}}
\def\ooy{\overline{\y}} \def\ooz{\overline{\z}}

\def\ooA{\overline{\A}} \def\ooB{\overline{\B}}
\def\ooC{\overline{\C}} \def\ooD{\overline{\D}}
\def\ooE{\overline{\E}} \def\ooF{\overline{\F}}
\def\ooG{\overline{\G}} \def\ooH{\overline{\H}}
\def\ooI{\overline{\I}} \def\ooJ{\overline{\J}}
\def\ooK{\overline{\K}} \def\ooL{\overline{\L}}
\def\ooM{\overline{\M}} \def\ooN{\overline{\N}}
\def\ooO{\overline{\O}} \def\ooP{\overline{\P}}
\def\ooQ{\overline{\Q}} \def\ooR{\overline{\R}}
\def\ooS{\overline{\S}} \def\ooT{\overline{\T}}
\def\ooU{\overline{\U}} \def\ooV{\overline{\V}}
\def\ooW{\overline{\W}} \def\ooX{\overline{\X}}
\def\ooY{\overline{\Y}} \def\ooZ{\overline{\Z}}

% vettoriali:

\def\va{\vec{\a}} \def\vb{\vec{\b}} \def\vc{\vec{\c}}
\def\vd{\vec{\d}} \def\ve{\vec{\e}} \def\vf{\vec{\f}}
\def\vg{\vec{\g}} \def\vh{\vec{\h}} \def\vib{\vec{\i}}
\def\vj{\vec{\j}} \def\vk{\vec{\k}} \def\vl{\vec{\l}}
\def\vm{\vec{\m}} \def\vn{\vec{\n}} \def\vo{\vec{\o}}
\def\vp{\vec{\p}} \def\vq{\vec{\q}} \def\vr{\vec{\r}}
\def\vts{\vec{\s}} \def\vtt{\vec{\t}} \def\vu{\vec{\u}}
\def\vv{\vec{\v}} \def\vw{\vec{\w}} \def\vx{\vec{\x}}
\def\vy{\vec{\y}} \def\vz{\vec{\z}}

\def\vA{\vec{\A}} \def\vB{\vec{\B}} \def\vC{\vec{\C}}
\def\vD{\vec{\D}} \def\vE{\vec{\E}} \def\vF{\vec{\F}}
\def\vG{\vec{\G}} \def\vH{\vec{\H}} \def\vI{\vec{\I}}
\def\vJ{\vec{\J}} \def\vK{\vec{\K}} \def\vL{\vec{\L}}
\def\vM{\vec{\M}} \def\vN{\vec{\N}} \def\vO{\vec{\O}}
\def\vP{\vec{\P}} \def\vQ{\vec{\Q}} \def\vR{\vec{\R}}
\def\vS{\vec{\S}} \def\vT{\vec{\T}} \def\vU{\vec{\U}}
\def\vV{\vec{\V}} \def\vW{\vec{\W}} \def\vX{\vec{\X}}
\def\vY{\vec{\Y}} \def\vZ{\vec{\Z}}

% cappello:

\def\ha{\hat{\a}} \def\hb{\hat{\b}} \def\hc{\hat{\c}}
\def\hd{\hat{\d}} \def\he{\hat{\e}} \def\hf{\hat{\f}}
\def\hg{\hat{\g}} \def\hh{\hat{\h}} \def\hib{\hat{\i}}
\def\hj{\hat{\j}} \def\hk{\hat{\k}} \def\hl{\hat{\l}}
\def\hm{\hat{\m}} \def\hn{\hat{\n}} \def\ho{\hat{\o}}
\def\hp{\hat{\p}} \def\hq{\hat{\q}} \def\hr{\hat{\r}}
\def\hts{\hat{\s}} \def\htt{\hat{\t}} \def\hu{\hat{\u}}
\def\hv{\hat{\v}} \def\hw{\hat{\w}} \def\hx{\hat{\x}}
\def\hy{\hat{\y}} \def\hz{\hat{\z}}

\def\hA{\hat{\A}} \def\hB{\hat{\B}} \def\hC{\hat{\C}}
\def\hD{\hat{\D}} \def\hE{\hat{\E}} \def\hF{\hat{\F}}
\def\hG{\hat{\G}} \def\hH{\hat{\H}} \def\hI{\hat{\I}}
\def\hJ{\hat{\J}} \def\hK{\hat{\K}} \def\hL{\hat{\L}}
\def\hM{\hat{\M}} \def\hN{\hat{\N}} \def\hO{\hat{\O}}
\def\hP{\hat{\P}} \def\hQ{\hat{\Q}} \def\hR{\hat{\R}}
\def\hS{\hat{\S}} \def\hT{\hat{\T}} \def\hU{\hat{\U}}
\def\hV{\hat{\V}} \def\hW{\hat{\W}} \def\hX{\hat{\X}}
\def\hY{\hat{\Y}} \def\hZ{\hat{\Z}}


==> trjcoms.tex <==
    \usepackage{latexsym}
\usepackage{subfigure}
\usepackage{amssymb}
\usepackage{url}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{psfrag}
%\usepackage{slashbox}

%impone di piazzare le figure prima del prossimo paragrafo (section)
\usepackage[section]{placeins}
\usepackage{arydshln}

%


 % \def\Ct{{\cos\{\theta\}}}
 % \def\St{{\sin\{\theta\}}}
\def\Ct{{c_\theta}}
\def\St{{s_\theta}}
\def\Cf{{c_\phi}}
\def\Sf{{s_\phi}}
\def\Cp{{c_\psi}}
\def\Sp{{s_\psi}}
\def\atan2{{\mbox{atan2}}}


% MACROS

\newcommand{\eq}[1]{eq.~(\ref{eq:#1})}
\newcommand{\Eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\eqn}[1]{(\ref{eq:#1})}
\newcommand{\Eqn}[1]{(\ref{eq:#1})}
\newcommand{\fig}[1] {fig.~\ref{fig:#1}}
\newcommand{\Fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\fign}[1] {\ref{fig:#1}}
\newcommand{\Fign}[1]{(\ref{fig:#1})}
\newcommand{\bib}[1]{~\cite{#1}}
\newcommand{\sez}[1]{Sez.~\ref{sec:#1}}
\newcommand{\sect}[1]{Sec.~\ref{sec:#1}}
\newcommand{\Sec}[1]{Sec.~\ref{sec:#1}}
\newcommand{\Section}[1]{Section~\ref{sec:#1}}
\newcommand{\ch}[1]{Chap.~\ref{ch:#1}}
\newcommand{\Chapter}[1]{Chapter~\ref{ch:#1}}
\newcommand{\tab}[1] {tab.~\ref{tab:#1}}
\newcommand{\Tab}[1] {Tab.~\ref{tab:#1}}

\newcommand{\bdot}[1] {\dot{\bf #1}}

\newcommand{\crx}[1]{{\bf #1}\times}
%-%\newcommand{\crx}[1]{{\bf S}({\bf #1})}
%\newcommand{\grad}[2]{\ {\bf grad}_{#2}(#1)\ }
%\newcommand{\hess}[2]{\ {\bf hess}_{#2}(#1)\ }
%-%\newcommand{\grad}[2]{\ \nabla_{#2}(#1)\ }
%-%\newcommand{\hess}[2]{\ {\bf H}_{#2}(#1)\ }
\newcommand{\grad}[2]{\frac{\partial #1}{\partial {#2}}}
\newcommand{\hess}[2]{\frac{\partial^2 #1}{\partial{\bf #2}^2}}
\newcommand{\bg}[1]{\mbox{\boldmath $#1$}}
\newcommand{\dt}[1]{\frac{d~#1}{dt}}

\def\fitem{\item[$\Rightarrow~$]}

\def\DEIS{Dipartimento di Elettronica Informatica e Sistemistica}
\def\DIEM{Dipartimento di Meccanica}


\def\12{\frac{1}{2}}

%\def\aa{\`a} \def\ee{\`e} \def\ii{\`{i}} \def\oo{\`o} \def\uu{\`u}

% \def\a{{\bf a}}
%  % \def\b{{\bf b}}
% \def\c{{\bf c}} \def\d{{\bf d}}
% \def\e{{\bf e}} \def\f{{\bf f}} \def\g{{\bf g}} \def\h{{\bf h}}
% \def\ib{{\bf i}} \def\j{{\bf j}} \def\k{{\bf k}} \def\l{{\bf l}}
% \def\m{{\bf m}} \def\n{{\bf n}} \def\o{{\bf o}} \def\p{{\bf p}}
% \def\q{{\bf q}} \def\r{{\bf r}} \def\s{{\bf s}} \def\t{{\bf t}}
% \def\u{{\bf u}} \def\v{{\bf v}} \def\w{{\bf w}} \def\x{{\bf x}}
% \def\y{{\bf y}} \def\z{{\bf z}}

% \def\A{{\bf A}} \def\B{{\bf B}} \def\C{{\bf C}} \def\D{{\bf D}}
% \def\E{{\bf E}} \def\F{{\bf F}} \def\G{{\bf G}} \def\H{{\bf H}}
% \def\I{{\bf I}} \def\J{{\bf J}} \def\K{{\bf K}} \def\L{{\bf L}}
% \def\M{{\bf M}} \def\N{{\bf N}} \def\O{{\bf O}} \def\P{{\bf P}}
% \def\Q{{\bf Q}} \def\R{{\bf R}} \def\S{{\bf S}} \def\T{{\bf T}}
% \def\U{{\bf U}} \def\V{{\bf V}} \def\W{{\bf W}} \def\X{{\bf X}}
% \def\Y{{\bf Y}} \def\Z{{\bf Z}}


\def\a{\mbox{\boldmath $a$}}  \def\b{\mbox{\boldmath $b$}}
\def\c{\mbox{\boldmath $c$}} \def\d{\mbox{\boldmath $d$}}
\def\e{\mbox{\boldmath $e$}} \def\f{\mbox{\boldmath $f$}} \def\g{\mbox{\boldmath $g$}} \def\h{\mbox{\boldmath $h$}}
\def\ib{\mbox{\boldmath $i$}} \def\j{\mbox{\boldmath $j$}} \def\k{\mbox{\boldmath $k$}} \def\l{\mbox{\boldmath $l$}}
\def\m{\mbox{\boldmath $m$}} \def\n{\mbox{\boldmath $n$}} \def\o{\mbox{\boldmath $o$}} \def\p{\mbox{\boldmath $p$}}
\def\q{\mbox{\boldmath $q$}} \def\r{\mbox{\boldmath $r$}} \def\s{\mbox{\boldmath $s$}} \def\t{\mbox{\boldmath $t$}}
\def\u{\mbox{\boldmath $u$}} \def\v{\mbox{\boldmath $v$}} \def\w{\mbox{\boldmath $w$}} \def\x{\mbox{\boldmath $x$}}
\def\y{\mbox{\boldmath $y$}} \def\z{\mbox{\boldmath $z$}}

\def\A{\mbox{\boldmath $A$}} \def\B{\mbox{\boldmath $B$}} \def\C{\mbox{\boldmath $C$}} \def\D{\mbox{\boldmath $D$}}
\def\E{\mbox{\boldmath $E$}} \def\F{\mbox{\boldmath $F$}} \def\G{\mbox{\boldmath $G$}} \def\H{\mbox{\boldmath $H$}}
\def\I{\mbox{\boldmath $I$}} \def\J{\mbox{\boldmath $J$}} \def\K{\mbox{\boldmath $K$}} \def\L{\mbox{\boldmath $L$}}
\def\M{\mbox{\boldmath $M$}} \def\N{\mbox{\boldmath $N$}} \def\O{\mbox{\boldmath $O$}} \def\P{\mbox{\boldmath $P$}}
\def\Q{\mbox{\boldmath $Q$}} \def\R{\mbox{\boldmath $R$}} \def\S{\mbox{\boldmath $S$}} \def\T{\mbox{\boldmath $T$}}
\def\U{\mbox{\boldmath $U$}} \def\V{\mbox{\boldmath $V$}} \def\W{\mbox{\boldmath $W$}} \def\X{\mbox{\boldmath $X$}}
\def\Y{\mbox{\boldmath $Y$}} \def\Z{\mbox{\boldmath $Z$}}


 % \def\qdot{\dot{\bf q}}
 \def\udot{\dot{\bf u}} \def\xdot{\dot{\bf x}}
\def\ydot{\dot{\bf y}} \def\ccdot{\dot{\bf c}} \def\pdot{\dot{\bf p}}
\def\vdot{\dot{\bf v}} \def\rdot{\dot{\bf r}}  \def\bddot{\dot{\bf d}}

 % \def\dotq{\dot{q}}
 \def\dotx{\dot{x}}

\def\0{{\bf 0}}

% CAL
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cM{{\cal M}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cU{{\cal U}}
\def\cT{{\cal T}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}

 %  \def\btau{{\bmit \tau}}
 %  \def\bphi{{\bmit \phi}}
 %  \def\bpsi{{\bmit \psi}}
 %  \def\bomega{{\bmit \omega}}
 %  \def\bgamma{{\bmit \gamma}}


 % Mathematic boldfaces
 %  \def\btau{{\makebox{\boldmath $\tau$}}}
 %  \def\bom{{\makebox{\boldmath $\omega$}}}
 %  \def\bomega{{\makebox{\boldmath $\omega$}}}
 %  \def\bphi{{\makebox{\boldmath $\phi$}}}
 %  \def\bpsi{{\makebox{\boldmath $\psi$}}}
 %  \def\balpha{{\makebox{\boldmath $\alpha$}}}
 %  \def\bbeta{{\makebox{\boldmath $\beta$}}}
 %  \def\bupsilon{{\makebox{\boldmath $\upsilon$}}}
 %  \def\bnu{{\makebox{\boldmath $\nu$}}}
 %  \def\b0{{\makebox{\boldmath $0$}}}

 \def\btau{{\mbox{\boldmath $\tau$}}}
 \def\bom{{\mbox{\boldmath $\omega$}}}
 \def\bomega{{\mbox{\boldmath $\omega$}}}
 \def\bphi{{\mbox{\boldmath $\phi$}}}
 \def\bpsi{{\mbox{\boldmath $\psi$}}}
 \def\balpha{{\mbox{\boldmath $\alpha$}}}
 \def\bbeta{{\mbox{\boldmath $\beta$}}}
 \def\bupsilon{{\mbox{\boldmath $\upsilon$}}}
 \def\bnu{{\mbox{\boldmath $\nu$}}}
 \def\b0{{\mbox{\boldmath $0$}}}

 \def\bA{{\mbox{\boldmath $A$}}}
 \def\bB{{\mbox{\boldmath $B$}}}
 \def\oB{\overline{\mbox{{\boldmath $B$}}}}
 \def\bC{{\mbox{\boldmath $C$}}}
 \def\oC{\overline{\mbox{{\boldmath $C$}}}}
 \def\bD{{\mbox{\boldmath $D$}}}
 \def\bI{{\mbox{\boldmath $I$}}}
 \def\bK{{\mbox{\boldmath $K$}}}
 \def\bL{{\mbox{\boldmath $L$}}}
 \def\bM{{\mbox{\boldmath $M$}}}
 \def\bP{{\mbox{\boldmath $P$}}}
 \def\oP{\ \overline{\mbox{{\boldmath $P$}}}}
 \def\bR{{\mbox{\boldmath $R$}}}
 \def\bO{{\mbox{\boldmath $0$}}}
 \def\oQ{\overline{\mbox{{\boldmath $Q$}}}}
 \def\bW{{\mbox{\boldmath $W$}}}
 \def\oW{\overline{\mbox{{\boldmath $W$}}}}
 \def\bX{{\mbox{\boldmath $X$}}}
 \def\bb{{\mbox{\boldmath $b$}}}
 \def\bet{{\mbox{\scriptsize \boldmath $e$}}}
 \def\bg{{\mbox{\boldmath $g$}}}
 \def\bm{{\mbox{\boldmath $m$}}}
 \def\bp{{\mbox{\boldmath $p$}}}
 %  \def\bps{{\mbox{\small \boldmath $p$}}}
 %  \def\bpf{{\mbox{\footnotesize \boldmath $p$}}}
 \def\bps{{\mbox{\scriptsize \boldmath $p$}}}
 \def\bpt{{\mbox{\tiny \boldmath $p$}}}
 \def\bq{{\mbox{\boldmath $q$}}}
 \def\bqt{{\mbox{\tiny \boldmath $q$}}}
 \def\bs{{\mbox{\boldmath $s$}}}
 \def\bt{{\mbox{\boldmath $t$}}}
 \def\bu{{\mbox{\boldmath $u$}}}
 \def\bx{{\mbox{\boldmath $x$}}}
 \def\bz{{\mbox{\boldmath $z$}}}

 \def\qdot{\dot{\bq}}

 % \def\l[{\left[}   \def\r]{\right]}
 % \def\l({\left(}   \def\r){\right)}
 % \def\op{\left\{}  \def\cb{\right\}}

 % \newcommand{\Rm}{{\sf R\hspace*{-0.9ex}\rule{0.15ex}%
 % {1.5ex}\hspace*{0.9ex}}}
 % \newcommand{\Nm}{{\sf N\hspace*{-1.0ex}\rule{0.15ex}%
 % {1.3ex}\hspace*{1.0ex}}}
 % \newcommand{\Qm}{{\sf Q\hspace*{-1.1ex}\rule{0.15ex}%
 % {1.5ex}\hspace*{1.1ex}}}
 % \newcommand{\Cm}{{\sf C\hspace*{-0.9ex}\rule{0.15ex}%
 % {1.3ex}\hspace*{0.9ex}}}

\newcommand{\Rm}{{\rm R\hspace*{-0.9ex}\rule{0.15ex}%
{1.5ex}\hspace*{0.9ex}}}
\newcommand{\Nm}{{\rm N\hspace*{-1.0ex}\rule{0.15ex}%
{1.3ex}\hspace*{1.0ex}}}
\def\natural{\mbox{\rm I\kern-0.2em N}}  % Symbol for the set of real numbers.
\newcommand{\Qm}{{\rm Q\hspace*{-1.1ex}\rule{0.15ex}%
{1.5ex}\hspace*{1.1ex}}}
% \newcommand{\Cm}{{\rm C\hspace*{-0.9ex}\rule{0.15ex}%
% {1.3ex}\hspace*{0.9ex}}}
\newcommand{\Cm}{{\sf C\hspace*{-0.9ex}\rule{0.15ex}%
       {1.3ex}\hspace*{0.9ex}}}
%\newcommand{\Cm}{\mathbb{C}}


%      \newcommand{\R}{{\sf R\hspace*{-0.9ex}\rule{0.15ex}%
%       {1.5ex}\hspace*{0.9ex}}}
%       \newcommand{\N}{{\sf N\hspace*{-1.0ex}\rule{0.15ex}%
%       {1.3ex}\hspace*{1.0ex}}}
%       \newcommand{\Q}{{\sf Q\hspace*{-1.1ex}\rule{0.15ex}%
%       {1.5ex}\hspace*{1.1ex}}}
%       \newcommand{\C}{{\sf C\hspace*{-0.9ex}\rule{0.15ex}%
%       {1.3ex}\hspace*{0.9ex}}}

 % \newcommand{\sf}[1]{\hspace{%1mm}\Lra\hspace{%1mm}}

\def\diag{\mbox{\sf diag $\;$}}
\def\real{\mbox{\rm I\kern-0.2em R}}  % Symbol for the set of real numbers.
\def\=def{\stackrel{def}{=}}
\def\wh{\noindent}
\def\ni{\noindent}
\def\nis{\hspace*{-1.5mm}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\beann{\begin{eqnarray*}}
\def\eeann{\end{eqnarray*}}

\def\ds{\displaystyle}
\def\sbf{\bf \sf}
\def\sit{\it \sf}
\newcommand{\fracd}[2]{\frac{\ds #1}{\ds #2}}

\def\vsp{\vspace*{5mm}}
\def\vspi{\vspace*{5mm}}
\def\vspii{\vspace*{10mm}}
\def\vspiii{\vspace*{15mm}}
\def\vspiiii{\vspace*{20mm}}
\def\hsp{\hspace*{5mm}}
\def\hspi{\hspace*{5mm}}
\def\hspii{\hspace*{10mm}}
\def\hspiii{\hspace*{15mm}}
\def\hspiiii{\hspace*{20mm}}

\def\ra{\rightarrow}
\def\Ra{\Rightarrow}
\def\Lra{\Longrightarrow}

\def\la{\leftarrow}
\def\La{\Leftarrow}
\def\Lla{\Longleftarrow}

\def\lra{\Leftrightarrow}
\def\Llra{\Longleftrightarrow}

 % \newtheorem{theor}{Theorem}
 % \newtheorem{claim}{Claim}
 % \newtheorem{algorithm}{Algorithm}
 % \newtheorem{definition}{Definition}
 % \newtheorem{lemma}{Lemma}
 % \newtheorem{prop}{Proposition}
 % \newtheorem{corollary}{Corollary}

\newenvironment{myeqnarray}%%
  {\setlength{\arraycolsep}{0.14em} %% 0.14em = 2.5/18 quad = 0.5 thickspace,
   \begin{eqnarray}}%%%                default value was 5 pt (much bigger)
  {\end{eqnarray}}           %% see The TeXbook, p. 167-170

%% Footnote on the first page %%
 %  \newcommand{\sedepubblicazione}[1]{%
 %    \begin{table}[b]       % e` una tabella in fondo alla pagina.
 %      \footnotesize
 %      \footnoterule        % tratto di separazione
 %     {#1}                  % testo della nota
 %     \end{table}
 %   }                       % fine definizione

%-----------------------------------------------------------------
% Defines a boxit environment, which draws lines around its contents.
% Usage:
%   \begin{boxit}
%       ... (text you want to be boxed, can contain other environments)
%   \end{boxit}
%
% The width of the box is the width of the contents.
% The boxit* environment behaves the same, except that the box will be
% at least as wide as a normal paragraph.
%
%                                               Marcel van der Goot
%                                               marcel@cs.caltech.edu
%

\def\Beginboxit
   {\par
    \vbox\bgroup
           \hrule height1pt
           \hbox\bgroup
                  \vrule width1pt \kern2pt %
                  \vbox\bgroup\kern2pt
   }
\def\Endboxit{%
                             \kern2pt
                             \vspace*{4pt}
                       \egroup
                  \kern2pt\vrule width1pt
                \egroup
           \hrule height1pt
         \egroup
   }

\newenvironment{boxit}{\Beginboxit}{\Endboxit}
\newenvironment{boxit*}{\Beginboxit\hbox to\hsize{}}{\Endboxit}

\newcommand{\cbox}[1]{
                        \begin{boxit}
                        #1
                        \end{boxit}
                        }
%%%% -------------------------------------------------------- %%%%


%%% ---- Per il libro di traiettorie

\def\WDT{0.47\textwidth}
\def\HWDT{0.25\textwidth}
\def\BWDT{0.7\textwidth}

\def\ds{\displaystyle}

 \newcommand{\preamble}[1]{
 \begin{center}
 \begin{minipage}{0.8\textwidth}
 {\small \sf
 #1

 \underline{\hspace{\textwidth}}
 \vspace{2mm}
 }
 \end{minipage}
 \end{center}
 }

 %\newtheorem{esemp}{Example}[chapter]

 \newcommand{\Esempio}[1]{
 \begin{esemp}
 {\rm  #1 }
 %  \hspace*{\fill} $\Box$ \\
 \hspace*{\fill} $\Box$ \\
 \end{esemp}
 }

 \newcommand{\putab}{\centerline{
     \parbox[c]{0.5\textwidth}{\hspace{0.25\textwidth}\small (a)}
     \parbox[c]{0.5\textwidth}{\hspace{0.25\textwidth}\small (b)}}}

 \newcommand{\puttimed}{\vspace{-1.5mm}\centerline{
     \parbox[c]{0.5\textwidth}{\hspace{0.25\textwidth}\small t}
     \parbox[c]{0.5\textwidth}{\hspace{0.25\textwidth}\small t}}}

 \newif\ifSmallFigure \SmallFiguretrue
 \ifSmallFigure
    \def\FIGT2{c:/usr/claudio/work/ucima/tlibro/tfigure1} %tanto non lo usa
 \else
    \def\FIGT2{c:/usr/claudio/work/ucima/tlibro/tfigure} %tanto non lo usa
 \fi

\def\sign{\mathrm{sign}}

\def\vq{{\bq}}
%\def\q{q}
 % \def\vel{\dot q}
 % \def\v{\dot q}

\def\yq{{y}}
\def\dotq{\dot{q}}
\def\ddotq{\ddot{q}}
\def\dddotq{q^{(3)}}
\def\ddddotq{q^{(4)}}

\def\ac{\ddotq}
\def\j{\dddotq}
\def\s{\ddddotq}

\def\t{t}
\def\tzero{t_0}
\def\tuno{t_1}
 % \def\bq{{\bf q}}
 % \def\bs{{\bf s}}
 % \def\bt{{\bf t}}

\def\qzero{q_0}
\def\quno{q_1}
 % \def\qzero{\texttt{q}_0}
 % \def\quno{\texttt{q}_1}

\def\vel{\texttt{v}}
 % \def\vel{v}
\def\vzero{\vel_0}
\def\vuno{\vel_1}
\def\vmax{\vel_{max}}
\def\vmin{\vel_{min}}
\def\hvmax{\hat \vel_{max}}
\def\hvmin{\hat \vel_{min}}

\def\deltav{\Delta V}
\def\deltaq{h}

\def\acc{\texttt{a}}
 % \def\acc{a}
\def\azero{\acc_{0}}
\def\auno{\acc_{1}}
\def\amax{\acc_{max}}
\def\amin{\acc_{min}}
\def\hamax{\hat\acc_{max}}
\def\hamin{\hat\acc_{min}}

\def\jerk{\texttt{j}}
 \def\snap{\texttt{s}}
 % \def\jerk{j}
\def\jzero{\jerk_{0}}
\def\juno{\jerk_{1}}
\def\jmax{\jerk_{max}}
\def\jmin{\jerk_{min}}
\def\hjmax{\hat \jerk_{max}}
\def\hjmin{\hat \jerk_{min}}
\def\szero{\snap_{0}}
\def\suno{\snap_{1}}

\def\smax{\snap_{max}}
\def\smin{\snap_{min}}

 % \def\alfa{\alpha}
\def\alfa{a}

\newcommand{\blambda}{\mbox{\boldmath$\lambda$}}
\newcommand{\bdelta}{\mbox{\boldmath$\delta$}}
 % \newcommand{\btau}{\mbox{\boldmath$\tau$}}

% Per sistemi discretizzati
\def\qd{\q_k}
\def\vd{\dotq_k}
\def\acd{\ddotq_k}
\def\jd{\j_k}
\def\sd{\s_k}

\def\qdm1{\q_{k-1}}
\def\vdm1{\dotq_{k-1}}
\def\acdm1{\ac_{k-1}}
\def\jdm1{\j_{k-1}}

\def\hq{\hat q}
\def\hv{\hat \vel}
\def\hac{\hat \acc}


\def\hdotq{\dot{\hat{q}}}
\def\hddotq{\ddot{\hat{q}}}
\def\hdddotq{{\hat{q}}^{(3)}}


\def\im{{\rm{j}}}

 \def\qn{{q _{\mbox{\tiny{$N$}}}}}% Traiettoria in forma normalizzata
 \def\tqn{\tilde q _{\mbox{\tiny{$N$}}}}% Traiettoria in forma normalizzata
 \newcommand{\qnpow}[1]{q ^{#1}_{\mbox{\tiny{$N$}}}}
 \newcommand{\tqnpow}[1]{\tilde q ^{#1}_{\mbox{\tiny{$N$}}}}
 \def\dqn{\dot q _{\mbox{\tiny{$N$}}}}
 \def\ddqn{\ddot q _{\mbox{\tiny{$N$}}}}

 \def\Vn{V_{\mbox{\tiny{$N$}}}}

 % \def\bM{\mathbf{\it \bf M}}


==> trjfilter2.tex <==
%\def\dy{\dot y}
%\def\ddy{\ddot y}
%\def\um{\dddot x_{\mbox{\tiny{m}}}}
%\def\uM{\dddot x_{\mbox{\tiny{M}}}}
%\def\dym{\dot y_{\mbox{\tiny{m}}}}
%\def\dyM{\dot y_{\mbox{\tiny{M}}}}
%\def\ddym{\ddot y_{\mbox{\tiny{m}}}}
%\def\ddyM{\ddot y_{\mbox{\tiny{M}}}}
%\def\umM{(\um-\uM)}
%%\def\umM{\ddot x_{\mbox{\tiny{mM}}}}
%\def\D{(\ddy^2 - 2\dy\uM)}

\def\dy{\dot y}
\def\ddy{\ddot y}
%\def\dddxm{\jerk_{\mbox{\tiny{m}}}}
%\def\um{\dddxm}
%\def\dddxM{\jerk_{\mbox{\tiny{M}}}}
%\def\uM{\dddxM}
%\def\ddxm{\acc_{\mbox{\tiny{m}}}}
%\def\ddxM{\acc_{\mbox{\tiny{M}}}}
%\def\dxm{\vel_{\mbox{\tiny{m}}}}
%\def\dxM{\vel_{\mbox{\tiny{M}}}}
%\def\dym{\dot y_{\mbox{\tiny{m}}}}
%\def\dyM{\dot y_{\mbox{\tiny{M}}}}
%\def\ddym{\ddot y_{\mbox{\tiny{m}}}}
%\def\ddyM{\ddot y_{\mbox{\tiny{M}}}}


\newcommand{\xM}[1]{\overline{x}_{#1}}
\newcommand{\xm}[1]{\underline{x}_{#1}}

\newcommand{\yM}[1]{\overline{y}_{#1}}
\newcommand{\ym}[1]{\underline{y}_{#1}}

\def\dddxm{\xm{0}}
\def\um{\dddxm}
\def\dddxM{\xM{0}}
\def\uM{\dddxM}
\def\ddxm{\xm{1}}
\def\ddxM{\xM{1}}
\def\dxm{\xm{2}}
\def\dxM{\xM{2}}
\def\dym{\ym{2}}
\def\dyM{\yM{2}}
\def\ddym{\ym{1}}
\def\ddyM{\yM{1}}

\def\umM{(\um-\uM)}
%\def\umM{\ddot x_{\mbox{\tiny{mM}}}}
\def\Dp{(y_1^2 - 2y_2\um)}
\def\Dm{(y_1^2 - 2y_2\uM)}

\def\uu{\hat u_1}
\def\ud{\hat u_2}
\def\udu{(\ud-\uu)}
\def\uud{(\uu-\ud)}

\def\Dd{(y_1^2 - 2y_2\ud)}
\def\Du{(y_1^2 - 2y_2\uu)}


